Constantine: Automatic Side-Channel Resistance Using Efficient Control and Data Flow Linearization

In the era of microarchitectural side channels, vendors scramble to deploy mitigations for transient execution attacks, but leave traditional side-channel attacks against sensitive software (e.g., crypto programs) to be fixed by developers by means of constant-time programming (i.e., absence of secret-dependent code/data patterns). Unfortunately, writing constant-time code by hand is hard, as evidenced by the many flaws discovered in production side channel-resistant code. Prior efforts to automatically transform programs into constant-time equivalents offer limited security or compatibility guarantees, hindering their applicability to real-world software. In this paper, we present Constantine, a compiler-based system to automatically harden programs against microarchitectural side channels. Constantine pursues a radical design point where secret-dependent control and data flows are completely linearized (i.e., all involved code/data accesses are always executed). This strategy provides strong security and compatibility guarantees by construction, but its natural implementation leads to state explosion in real-world programs. To address this challenge, Constantine relies on carefully designed optimizations such as just-in-time loop linearization and aggressive function cloning for fully context-sensitive points-to analysis, which not only address state explosion, but also lead to an efficient and compatible solution. Constantine yields overheads as low as 16% on standard benchmarks and can handle a fully-fledged component from the production wolfSSL library.

==> notes.tex <==
backend% !TEX root = main.tex

\section{Old Notes}
\dan{All the text below was written early during Cristiano's visit, it's meant to be only a collection of bib entries really. Don't judge me :-P}

Classic side-channel attacks build on information gained from the implementation of a computation rather than on theoretical weaknesses of algorithms. An attacker may observe a computation at different levels, including the kind of instruction executed every instant, the amount of time required by each such instruction, and even which addresses in memory it reads from or writes to. Caches, branch predictors, and memory address traces are examples of side-channels regularly exploited in the literature.

One way to protect code against such attacks is to deploy implementations that have {\em constant} ``observable'' effects for any input: that is, an attacker cannot distinguish two executions under two arbitrarily different inputs, which limits their wiggle room to mount a side-channel attack. The popular {\em constant-time programming} abstraction requires to this end the control flow and the memory accesses to be independent from secret data.

Unfortunately, writing constant-time code is no small feat: timing leaks repeatedly disclosed in popular cryptographic libraries suggest that the research community has at least two aspects to address with practical solutions that are strong in a security sense. The first is the need for tools for validating constant-time implementations: analysis at source-code or compiler-representation level (e.g., ~\cite{ctverif-SEC16}) should be complemented with binary-level verification tools as shown recently in~\cite{binsecrel-SP20}. The second is a heartfelt necessity of tools that can aid developers in writing constant-time implementations in the first place.

We propose a solution that can help in retrofitting existing software implementations and performing program repair for flawed constant-time code. {\sc ConstantTine} builds around two main concepts:
\begin{itemize}
\item {\em control-flow linearization}, [...]
\item {\em data-flow linearization}, [...]
\end{itemize}

\noindent
Technical items:
\begin{itemize}
\item {\em dummy mode} idea
\item CFG flattening
\item indirect call promotion
\item profiling stage + taint-driven linearization
\item function outlining for tainted branches
\item everything expressed at compiler IR level, but also avoiding distortions in the backend that can happen as pointed out in~\cite{binsecrel-SP20}
\end{itemize}

\noindent
Compared to previous proposals, {\sc ConstantTine} advances the state of the art in several respects: 
\begin{itemize}
\item loops
\item function calls (?)
\item data-flow linearization instead of Path-ORAM or SGX
\item indirect memory references {\em (erm, let's rephrase this...)}
\item dependencies from nesting and implicit dependencies (?)
\item {\em what else?}
\end{itemize}


\subsubsection*{Prior Works}
\begin{itemize}
\item (ICISC'05) {\em The Program Counter Security Model: Automatic Detection and Removal of Control-Flow Side Channel Attacks}~\cite{Molnar-ICISC05}
\item (Oakland'09) {\em Practical Mitigations for Timing-Based Side-Channel Attacks on Modern X86 Processors}~\cite{Coppens-SP09}
\item (TACO'12) {\em Compiler Mitigations for Time Attacks on Modern x86 Processors}~\cite{vanCleemput-TACO12}
\item (USENIX SEC'15) {\em Raccoon: Closing Digital Side-Channels through Obfuscated Execution}~\cite{RACCOON-SEC15}
\item (ISSTA'18) {\em Eliminating Time Side-Channel Leaks using Program Repair}~\cite{Wu-ISSTA18}
\item (TDSC'20) {\em Adaptive Compiler Strategies for Mitigating Timing Side Channel Attacks}~\cite{vanCleemput-TDSC20}
\end{itemize}

\noindent{\small\bf\em TODO}
\begin{itemize}
\item Language-Based Control and Mitigation of Timing Channel (PLDI'12)~\cite{Zhang-PLDI12}
\item Constant-Time Foundations for the New Spectre Era (PLDI'20)~\cite{Cauligi-PLDI20}
\end{itemize}

\subsubsection*{References for Concepts}
\begin{itemize}
\item program counter security model~\cite{Molnar-ICISC05}
\item design of modern processors (e.g. load bypassing, register renaming)~\cite{Shen-2005book}
\item if-conversion~\cite{Allen-POPL83}, efficient predicated execution~\cite{August-ISCA99}, predicate speculation~\cite{Schlansker-PLDI99}
\item micro-architectural side channels of branch prediction, instruction caching, and branch target buffers {\em (works by Acii\c{c}mez cited in \cite{vanCleemput-TACO12} -- TODO: look for other/more relevant ones)}
\item early-terminating multiplication~\cite{Groundefin-ICISC09}, variable latency instructions on x86~\cite{Coke08-ITJ08, Fog-TR11,Granlund-TR12}, abnormalities with floating point instructions~\cite{Andrysco-SP15} and techniques to achieve constant-time FP computations~\cite{CFTP-CCS18}
\item processor concepts: optimistic and pessimistic load bypassing, store forwarding, 4K aliasing, memory disambiguation (conflict speculation), alignment, partial aliasing, bank conflicts {\em (\cite{vanCleemput-TACO12} only mentions them...)}
\item mutual information analysis to detect correlations for attacks~\cite{Gierlichs-CHES08, Batina-JC11, Whitnall-CRYPTO11}
\item attacks based on contention for shared resources~\cite{Wang-ISCA07, Hunger-HPCA15}
\item Path ORAM~\cite{PATHORAM-CCS13, PATHORAM-JACM18} and other ORAM papers~\cite{ASCEND-STC12, PHANTOM-CCS13}
\item memory trace obliviousness~\cite{MTO-CSF13} by GhostRider~\cite{GHOSTRIDER-ASPLOS15}
\item limit leaks from loop trip counts and recursive calls~\cite{Zhang-CCS11}
\item PL techniques for detecting/proving absence of timing leaks~\cite{Antonopoulos-PLD17, Chen-CCS17, Sousa-PLDI16}
\item cache side channels {\em (\cite{Wu-ISSTA18} cites a bunch of papers)}
\item equalizing branches by cross-copying~\cite{Agat-POPL00, Kopf-IJIS07, Kopf-FAST05, Molnar-ICISC05} {\em (flaws discussed in \cite{Wu-ISSTA18} and \cite{Mantel-ESORICS15}, this line of work seems behind the works by Molnar et al. but Agat originally introduced type-driven cross-copying)}
\item field-sensitive points-to analysis~\cite{Balatsouras-SAS16, Pearce-PASTE04}
\item constant-time binary level verification~\cite{binsecrel-SP20}
\end{itemize}


==> related.tex <==
% !TEX root = main.tex
\section{Other Related Works}
\label{se:related}

We described prior solutions in \textsection\ref{se:background} and drew comparisons as we discussed our design. This section covers other related literature. % related to our work.

\textcolor{magenta}{
\begin{itemize}
\item leak analysis
\item type-based solutions, hw stuff
\item obfuscuro and SGX-related stuff
\item what else?
\end{itemize}
}

==> scratchpad.tex <==
In addition to handling full expressivity for loop constructs, compared to prior approaches \proj does not require static unrolling: this not only allows us to handle trip counts that diverge from an oracle's prediction (using extremely conservative upper bounds would introduce too many decoy paths that kill performance~\cite{SomeWork}), but also to keep the code size compact: this paves the way to further compiler optimizations, such as inlining, that Soares et al. observe would make linearization unpractical when combined with unrolling~\cite{cgo21}. \dan{stretched; rewrite}\pie{about unrolling: cannot dynamically fix max\_count misprediction once unrolled, we can instead. Sometimes you cannot unroll as the value would be too big: e.g. what if max\_count=1.000.000}

With our selective cloning, we trade context sensitivity for code size, allowing our programs to ship hard-wired DFL metadata information for the allocation sites and the possible access patterns over the abstract objects from the points-to analysis. We opted for this choice as we believe it can bring a lower run-time overhead than an alternative design that merges the cloned functions after the points-to analysis and maintains a shadow call stack, selecting which DFL metadata to use depending on the current calling context of a function making a sensitive memory access. This design could be used however in deploy targets that are sensitive to code size. In that respect, our loop handling significantly outperforms prior designs as we can avoid costly unrolling of loop bodies.\dan{Thoguhts? I'm trying to prevent criticism on e.g. low-performance devices}

\dan{shall we emphasize portability?}

\dan{Left out: array sensitivity, C++ code vs indirect calls}

\dan{TODO} By adding context-sensitivity we reduce the number of objects to work on, and by improving field-sensitivity we reduce the sizes involved in the striding process.


%%%%%%
Another relevant feature of our oracle is how we enhanced the field-sensitivity analysis of SVF. Field sensitivity implies that a points-to analysis can distinguish different fields of the same abstract object. This aspect is crucial for the efficiency of DFL, as we want to minimize for the sake of completeness (and ultimately performance) the amount of memory operations: real-world crypto code uses many-field, nested data structures of hundreds or thousands of bytes, and in the entire execution a load or store operation may dereference only a limited portion of them.

\dan{I think the problem here may be that in unoptimized code you may have field info, but unoptimized code is hard to work on for us? Or is there some weird pointer arithmetics that makes SVF go crazy? I am asking before we mention ugly GEPs and other effects from optimization.}\pie{purtroppo e' tosta dire esattamente cosa fa impazzire SVF ogni tanto e non farei risky guesses, uglygep sicuro, ma anche pointer arithmetics o simili}~\dan{how does it look now? you still think it's unsafe? I feel that not giving a motivation could be equally bad for reviewers. We should also look up the literature}

We observed that for our wolfSSL case study the field-sensitive Andersen implementation of SVF fails to recover field information for a very large fraction (over $90\%$) of the secret-dependent accesses, returning the whole object as potentially dereferenced. In our analysis pointer arithmetics in the code seems to be a main cause that makes SVF fall back to field-insensitive abstract objects, and compiler optimizations exacerbate this issue. % ~\dan{PB got a ballpark estimate? 30-50\%?}\pie{25\% con la enhanced SVF che non promuove objects a field insensitive, prima con la github version era peggio, tipo 90\%}

%%%%%%
In alias analysis research for Java programs, Whaley and Lam~\cite{whaley-pldi04} create a function clone for every distinct calling context, use binary decision diagrams to handle the large number of contexts after cloning, and use Datalog to implement a context-insensitive points-to analysis than gives context-sensitive results thanks to cloning.

turn a context-insensitive points-to analysis into a context-sensitive one through cloning: they 

. The idea is to generate multiple instances of a function such that every distinct calling context invokes a different instance of the function. A calling context\footnote{The sequence of functions that are concurrently active on the stack~\cite{delia-spe16}.}  can be modeled as an acyclic path on the call graph~\cite{whaley-pldi04}: whenever a high number of such paths may make cloning impractical, an analysis can combine it with binary decision diagrams to model context-sensitive relations in a scalable manner.

\dan{Somewhere in the other oracle section (as well as in the introduction) we should say that on large code bases only some portions require linearization, to keep things practical.}

Our scenario however is special, as we may clone only the functions identified as secret-dependent by the other oracle, along with their callees, recursively. Hence we selectively clone along each maximal subtree of the call graph having a secret-dependent function as root. In this way, we obtain more accurate points-to sets for the load and store operations that undergo DFL, refining which abstract objects they can dereference for different calling contexts.

\iffalse %% will soon move in scratchpad.tex
\dan{PB help me out here, I may have written some BS}
One may wonder if also the analysis of allocation sites may benefit from cloning. In the crypto code we analyzed for this paper, after our selective cloning we tried to apply cloning also along call graph paths leading to allocation sites, and even to the whole code base, without obtaining more accurate points-to sets. Hence, we can conclude that selective cloning mimicked full context-sensitivity in the analysis of memory operations that had to undergo DFL.\pie{mmm mi sembra un po' risky come ragionamento, e non so se e' worth discussing, anche perche' non e' vero nel caso generale}

%we observed that the allocation sites for the objects composing the points-to sets above 
%are context-insensitive. In fact, repeating the analysis after applying cloning along the call graph paths leading to the functions that host the allocations (or even to the whole code base) does not yield smaller points-to sets. %Hence, we can conclude that selective cloning for secret-dependent functions allows us to obtain context-sensitivity for an inclusion-based points-to analysis.

%As calling context, we consider the sequence of functions that are concurrently active on the stack~\cite{delia-spe16}.
\fi


%%%%%
\dan{We won't implement this for CCS, so we will drop it}
The second strategy, which we call {\em dummy-aware linearization}, can reduce the size of the output list as it analyzes the behavior of the program along both real and decoy paths. This analysis is possible as CFL operates through indirection on the IR representation, hence we can re-run DFSan on the CFL-ed code by marking an IR virtual register as a taint source when assigning it during dummy execution (also note that we do not need to taint memory because decoy paths cannot alter it). With this strategy we linearize each nested construct for case (i) only if its decoy paths can leak: this choice preserves soundness and improves completeness. In \textsection\ref{se:case-study} we will see the practical benefits of this proposal on real-world code.

%%%%%%
Along with the address $p$ to dereference, which can be a pointer along a real path or $\bot$ (Figure~\ref{fig:dummy-addrs}), we pass the head of a doubly-linked list containing information on which object(s) it can reference. Such linked lists are initialized at compile time, and the program itself can update them upon e.g. dynamic memory (de)allocation.

\dan{We should explain how we obtain base and offset from p. To complete this part I need info on how striding happens and discuss cache lines vs addresses with PB. We will need a call :-)}

For a load operation, we use AVX-512 instructions to pull all the cache lines from the potential target objects in the linked list, and conditionally select the value that when the object enclosing $p$ is met. Along decoy paths {\tt ct\_load} always receives $\textrm{p}=\bot$, hence no real object address will match it: after touching all objects, we make the wrapper return a constant value (e.g. zero) of the desired size.

For a store operation, we break it into a load followed by a store. The rationale behind this choice is that only one memory location requires an update, but for linearization purposes we shall write to every plausible location from the points-to analysis or we would leak the target address. Hence for every involved location we read the current value, and replace it with the IR virtual register contents supplied for the store only when the location matches $p$, otherwise we write the current value back to memory. Hence decoy paths simply ``refresh'' the contents of every object, and real paths alter only one object while nonetheless writing to all of them.

\vspace{-1em}\textcolor{magenta}{
\begin{itemize}
\item optimized implementations for different sizes
\item AVX alternatives?
\end{itemize}
}


%%%%%%


Once we dealt with side channels from control flow decisions, we still need to address instructions whose latencies depend on the value of their operands, or on previous computation occurrences~\cite{oakland09}.

During the IR normalization step of \textsection\ref{ss:ir-norm}, we transform indirect calls into direct ones for two reasons: depending on the decisions of the oracle on which program regions require linearization (\textsection\ref{ss:taint}) we may need to linearize the callee as well, and we remove the effects of indirect call target prediction. As we discuss in \textsection\ref{ss:points-to}, for each call site we obtain a list of target candidates and replace the indirect call with an if-else series of direct calls, ended by a failsafe. 

During normalization we also replace LLVM instructions {\tt *div} and {\tt *rem} to use software counterparts that execute in constant time. Prior literature makes a similar decision, with the exception of~\ref{taco12} that explores multiplexing different division sequences for the 6 latency classes of the Core 2 micro-architecture, which can perform much faster than a software implementation but incurs limited portability, as each micro-architecture may require an ad-hoc formulation. \proj could be extended to do so whenever the user decides to produce code for a specific micro-architecture.

\dan{Remember: branch prediction for loop!!}
%%%%%%

Prior literature struggles with loops that depend on secret data. A few works provide partial support by trying to automatically infer a maximum trip count and pad the loop body with decoy paths for when the actual count is lower, then unroll it. Unrolling can also lead to code bloat.

These solutions typically do not support break and continue statements, nor they allow loop-computed variables to outlive the loop and later be used in the code. Let us consider the following sensitive fragment from the wolfSSL library:
\dan{Check limitations; add references to specific works? mention code bloat}


\begin{center}
\begin{lstlisting}[language=C, style=inlineCode]
/* now copy out */
_c   = c + pa;
tmpm = a->dp;
for (x = 0; x < pa+1; x++)
  *tmpm++ = *_c++;
/* zero any excess digits on destination that we didn't write to */
for (; x < oldused; x++)
  *tmpm++ = 0;
\end{lstlisting}
\end{center}

The code computes $x/R == x~(mod~N)$ using a Montgomery reduction. The induction variable of the first loop outlives it and dictates the trip count of the second loop. Also, we found many instances of continue and break statement in wolfSSL. 

% or they lament large code sizes after unrolling that  (Soares)


\subsubsection{Dummy Execution}
\label{ss:dummy}
Before describing branch and loop linearization in detail, we present how CFL handles decoy computations. During the execution a linearized function maintains a \textit{``taken''} predicate to reflect whether the original program on the current program state would execute the next instruction (\textit{real path}) or not (\textit{decoy path}). We incrementally update this predicate at each linearized branching condition that guards a single-entry, single-exit region, and restore it upon leaving the region. Thanks to this predicate, we realize a {\em dummy execution} abstraction such that computations from decoy paths cannot pollute the program state, neither can crash the program nor make bogus memory operations.

The key to correctness is that we can safely allow decoy paths to make local computations (i.e. assign to SSA virtual registers), as long as their values do not flow into memory operations or other instructions (e.g. division) that can lead to exceptions.

For memory operations, each pointer expression computation conditionally selects an artificial $\bot$ value when in dummy execution, then as we will see in \textsection\ref{se:dfl} the DFL load and store primitives prevent data-dependent leaks for both real and decoy paths thanks to points-to metadata associated with the memory operation.

\paragraph{Motivation}
Table~\ref{tab:comparison} depicts the state of the art of compiler-based defenses for digital side channels. In terms of supported language expressivity \leo{perché ``expressivity''?}\dan{vedi ora se ok}, each solution may struggle with: loops with secret-dependent trip counts, indirect function calls, dynamic memory allocation, and variable-size or multi-dimensional objects dereferenced at memory accesses. No solution can at the same time preserve security and execution correctness and handle the memory layout and access patterns typical of complex real-world code.\dan{drop complex?}% In terms of security, <= dropped

\dan{At some point we should say with blocked caches and random cache addressing are a no go right? We should also define decoy paths, maybe in the introduction so we can reuse it also for other works.}

Molnar et al.~\cite{Molnar-ICISC05} do not handle data-dependent side channels. Coppens et al.~\cite{Coppens-SP09} add protection for variable-latency instructions and solve correctness issues of~\cite{Molnar-ICISC05} with a \textit{cmov}-alike multiplexer, leaving data cache flows to orthogonal protection mechanisms like blocked caches and random cache addressing~\cite{xxx,yyy}. Raccoon~\cite{RACCOON-SEC15} uses a facility based on \textit{setjmp() - longjmp()} to linearize control flow, and a transaction mechanism based on a software implementation of a Path ORAM to let both real and decoy flows access and update memory. SC-Eliminator~\cite{Wu-ISSTA18} uses a \textit{cmov}-alike multiplexer for control flows, and preloads cache lines using a must-hit analysis to ensure that memory accesses do not incur cache misses.

Both Raccoon and SC-Eliminator can incur memory safety violations when dereferencing memory along decoy paths, which can result into termination leaks or accessing valid memory not belonging to the intended object. A very recent work~\cite{Soares-CGO21} points out that loads can go out of bounds because decoy paths would access addresses otherwise guarded by secret data. We came independently to a similar and possibly more general conclusion: decoy paths can induce arbitrary pointer expressions that both~\cite{RACCOON-SEC15} and~\cite{Wu-ISSTA18} dereference in their execution model, as they access an address\pie{mention access a ptr to ptr?}\dan{see next paragraph} and conditionally update a program state value: even if such value  is ultimately correct (i.e. the value from the decoy path is discarded with a \textit{cmov}), the invalid access still takes place and is observable.  

\dan{We also have indirection through memory to break Raccoon? Is it already captured by what I wrote above or shall we extend it?}

% WRONG? , nor pointers that over different invocations can refer to different arrays
Soares et al.~\cite{Soares-CGO21} propose a scheme that is alike to SC-Eliminator for obtaining straight-line code, and adds contracts to transformed code where the caller specifies the length of the presently accessed array. Contracts build on annotations at call sites obtained with a range analysis on top-level pointers that can reference an array: unfortunately, they do not support pointers obtained by dereferencing other pointers. When an access is outside the bounds or the bound could not be inferred, the scheme accesses a shadow variable instead of the address computed by the decoy path. However, accessing a shadow variable can be a side channel, and also introduce timing variations based on object strides as observed in~\cite{Coppens-SP09,vanCleemput-TACO12}.

Hence, we believe \proj can make a timely contribution to the state of the art as it brings expressivity and security guarantees that are not met to a similar extent by prior works.\leo{Qui forse dovremmo essere più convincenti. in pratica stiamo dicendo al reviewer che noi fixiamo le cose sbagliate presenti nelle altre soluzioni, ma non gli offriamo alcuna garanzia che non ci siano altre issues che non prendiamo in considerazione. La precedente affermazione per me si legge un po' come ``incremental work''}\dan{modifico in next revision}

\dan{Say something more on loop efficiency? Or perhaps later?}

\paragraph{Threat Model} In this paper we consider adversaries with the following capabilities and resources:
\begin{itemize}
\item they have access to the protected binary;\dan{source?}
\item they can probe the CPU instruction pointer value up to an instruction-level granularity;
\item they can run arbitrary code on the machine alongside the protected binary, even on the same core (hyperthreading siblings included) where the binary is executing;
\item they can monitor memory access timing and address traces.\dan{We need a discussion here: Raccoon considers an adversary that can inspect the whole stream of data accesses} 
\end{itemize}
% . Do we want to settle for cache lines as main adversary? Discuss the 1-byte/word-size striding separately?

% They can also attempt Spectre-like attacks, while Meltdown-like attacks are outside the threat model.\dan{Shall we say port contention and memjam upfront? How do we generalize that? See below}
We assume that the CPU is a sealed chip (Spectre, Meltdown, and MDS attacks fall outside the threat model) and the OS is trusted. Our adversary can attempt cache attacks of the likes of Flush+Reload, Prime+Probe, and others to influence memory access timings. They can observe memory at cache line granularity (an assumption used in constant-time crypto implementations) or at a more fine-grained one, as explored by CacheBleed~\cite{cachebleed} and MemJam~\cite{memjam} attacks.

Regarding the programs we seek to protect, like prior literature we assume that they are error-free: namely, it does not contain bugs that can lead to crashes or memory safety violations (e.g. out-of-bounds accesses), and it does not exhibit undefined behavior. Also, we assume that the program cannot leak secret data through external libraries, whose implementation is not visible to \proj.

Analog side channels like power consumption or EM radiation are outside the threat model and require orthogonal mitigations.\dan{What about resource contention attacks?} Whenever the adversary may monitor memory contents, the user can complement \proj with SGX or memory encryption mechanisms. 

\iffalse
\vspace{-1em}\textcolor{magenta}{
\begin{itemize}
\item can run code alongside the protected application (like Raccoon): so P+P, F+R, etc. + observation mechanisms for caches
\item the OS is trusted and so is the CPU chip
\item we do not consider an attacker targeting micro-architectural features like load ports of the CPU (no attack known yet, or it calls for new defenses and ours are still very relevant?)\pie{teoreticamente proteggiamo anche su port contention e memjam, meglio dire che non consideriatmo meltdown like attacks?}
\item what about data encryption and integrity of read/writes?
\item programs must be error-free, not only crash-free :)
\end{itemize}
}
\fi

%Shadow variable

\iffalse
\vspace{-1em}\textcolor{gray}{
\begin{itemize}
\item assumptions on programs (e.g. crash-free) and what we support
\item rule out attacks that target CPU core internals (i.e. uarch fun) and analog side channels (e.g. power)
\item mention flush+reload and other stuff not covered by ISSTA? will they expect an attack PoC?
\item provide an overview of the indirection approach (which impacts the organization of the paper too)
\item properties that \proj provides: PC security + no variable latencies from control flow (watch out for loops!), constant stream of data addresses
\end{itemize}
}
\fi


\begin{subfigure}[b]{0.27\columnwidth}
\centering
\begin{tabular}{c}
\begin{lstlisting}[style=myVerbatimStyle]
if (c) {
  a$_1$ = a$_0$+2
  b$_1$ = v[a$_1$]
}
b$_{4}$ = $\phi$(b$_1$,b$_0$)
if (!c) {
  b$_2$ = v[0]
}
b$_3$ = $\phi$(b$_2$,b$_{4}$)
\end{lstlisting}
\end{tabular}
\caption{if-Conversion\label{fig:cfl-b}}  
\end{subfigure}%

% discorso del nesting...
At this point we can further split a structure of the likes \textit{if (cond) then \{A\} else \{B\};} into two adjacent sequences \textit{if (cond) then \{A\};  if (!cond) then \{B\};} realizing what the compiler literature defines as \textit{if-conversion}~\cite{compiler-book}. Figure~\ref{fig:cfl-a} and~\ref{fig:cfl-b} depict an example of if-conversion~\pie{if-conversion now fixed to keep if/else regions}.

Based on the dummy execution abstraction that we described, we can remove the conditional branches to blocks A and B, link the blocks in an entry-A-B-exit fashion in the CFG, modify occurrences of memory load and store operations to choose their targets conditionally, and replace the $\phi$-nodes to keep the SSA representation well-formed.


%When the program reaches instructions corresponding to a basic block in the normalized CFG, it can access a ``taken'' boolean expression reflecting whether the original program would execute the block. This expression is a composition of one or more of the branching conditions defined in the single-entry, single-exit normalization step. To ensure that every such predicate holds a correct value according to the program semantics and that computations from decoy paths do not pollute the program state, we introduce a {\em dummy execution} abstraction.


\iffalse
 that ensures that every such predicate holds a correct value according to the program semantics, and that its memory .

Computations that involve local variables (i.e. IR virtual registers) can execute regardless, as they 

thanks to the single-entry-single-exit transformation we implicitly have a ``taken'' predicate reflecting whether the (original) program should execute the block. We introduce a {\em dummy execution} mode that ensures that every such predicate holds a correct value for the program semantics. When a block is in taken state, it can compute and update both local variables (i.e., IR virtual registers) and memory locations. When instead it is not, the 

To make sure that the predicate holds a correct value, computations that involve local variables (i.e., IR virtual registers) should propagate their results to later uses in the code

, the block is guarded by a ``taken'' predicate reflecting the branching decision in the original program, i.e., it determines whether we are on a real or a decoy path. For the latter case, we make sure that the computations that involve local variables (i.e., IR virtual registers) do not affect the real program state: upon leaving 
\fi
